Aggregating Layers for Deepfake Detection

The increasing popularity of facial manipulation (Deepfakes) and synthetic face creation raises the need to develop robust forgery detection solutions. Crucially, most work in this domain assume that the Deepfakes in the test set come from the same Deepfake algorithms that were used for training the network. This is not how things work in practice. Instead, we consider the case where the network is trained on one Deepfake algorithm, and tested on Deepfakes generated by another algorithm. Typically, supervised techniques follow a pipeline of visual feature extraction from a deep backbone, followed by a binary classification head. Instead, our algorithm aggregates features extracted across all layers of one backbone network to detect a fake. We evaluate our approach on two domains of interest - Deepfake detection and Synthetic image detection, and find that we achieve SOTA results.

==> 08_authors_response.tex <==
\section{Author's Response}
We thank the reviewers for their comments and efforts towards improving our manuscript. We edited the paper accordingly.

Recall that we propose an analysis network that runs on top of a standard backbone network such as EfficientNet-Small-V2 for Deepfake detection. The key insight is to aggregate features from all layers of the backbone before making the decision. We demonstrate that the method perform well both in detecting Deepfake, as well as detecting synthetic images. We compare our method to multiple other methods on multiple datasets and aggregate results using the Coefficient of Variance (CoV) measure. We achieve SOTA results according to this measure.

In addition, we have added a new section (Section~\ref{sec:Applications} that offers two possible applications of our Deepfake detection network. Specifically, we show two use cases. In the first, we show that it is possible to learn from the network activations which regions in the image are responsible to the decision if the image is real or fake. In the second use case, we show how we can trim $95\%$ of the number of parameters in our analysis network with negligible degradation in performance. 

Below is our deteiled response to comments made by the reviewers:

\textbf{Reviewer 1:}

Comment: \textit{Aggregating features from intermediate layers for enlarging the receptive field and improving representation is NOT novel enough.} 

Answer: Our method automatically finds the layers in the backbone network that capture most of the information if an image is real or fake. We further show how these layers can be mapped back to the image plane to show the regions that are suspected as being fake. Furthermore, we discuss ways to trim the analysis network, as mentioned above.

Comment: \textit{The accuracy of the proposed algorithm is better than others, but computation cost is unknown in the paper. Computation cost and number of parameters are also important for readers.}

Answer: The Applications~\ref{sec:Applications} section shows how with little / no additional parameters over the size of EfficientNet-V2, one can reach SOTA results.


Comment: \textit{The paper should be further polished for publication: the second paragraph of the introduction is too long. These information are not important for your paper.}

Answer: Deepfakes is a manipulation in which context disagrees with the face. Neural Textures, on the other hand, changes facial expression - this necessitates the measurement of lower level pixel statistics. We would like to refer the reviewer to Figure~\ref{fig:DeepfakesAnalysis}.  In figure Figure~\ref{fig:DeepfakesAnalysis}, we demonstrate how our method found this automatically.

Comment: \textit{"Code will be released upon acceptance. Is upon acceptance really necessary?"}

Answer: We will publish our code.

Comment: \textit{"In addition, we outperform a model created by taking EfficientNet-V2 and attaching a binary classification head on top of its 1000 soft class prediction outputs. We let the latter train end-to-end.”  Could you add there results to the tables?}

Answer: Added to Table~\ref{tab:SyntheticImagesAveragePrecisionWithCoV}.


\textbf{Reviewer 2:}

We thank the reviewer for the encouraging comments.

\textbf{Reviewer 4:}

Comment: \textit{My main concern is about the contribution of this paper.  The proposed method is too simple without any motivation/insight or explanation that why it is designed in this way.}

Answer: Aggregating allows the network to automatically pick the features needed for detecting fake or synthetic images. We added a new section that highlights two use cases that can benefit from our method. See discussion at the beginning of the page.

Comment: \textit{Besides, in some datasets, the proposed method didn't actually get SOTA results.}

Answer: In cases where the same algorithm needs to be ranked across numerous 'contests' (tests), it might be ambiguous to rank algorithms without a defined metric (other than the case when there is a winner who takes it all). We suggest to use the $CoV^{-1}$ metric, instead of Average Precision per task. For this metric we rank SOTA.


\textbf{Associate Editor:}

Comment: \textit{The AE agrees with both R1 and R4 that the proposed method is straightforward and the technical presentation needs some improvement.}

Answer: We upgraded the technical presentation and added the Applications~\ref{sec:Applications} section to better explain our contribution and method.



==> Tables/DeepfakeTables.tex <==
\begin{table*}[]

\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{Train on Deepfakes}} & \multicolumn{4}{|c|}{\textbf{Train on Neural Textures}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} \\
\hline
\hline
Resnet Layer 1 & 98.97 & 74.99 & 71.74 & 57.15 & 70.32 & 86.93 & 65.04 & 52.3 \\
Xception Block 1 & 92.95 & 70.52 & 65.94 & 52.83& 66.30 & 80.72 & 62.65 & 52.0 \\
Xception Block 2 & 98.04 & 70.28 & 67.48 & 56.04 & 69.31 & 85.75 & 64.27 & 52.7 \\
Xception Block 3 & 99.41 & 67.58 & 63.62 & 57.97 & 67.62 & 85.44 & 60.71 & 52.0\\
Xception Block 4 & 99.14 & 68.91 & 70.36 & 58.74 & 73.65 & 90.97 & 60.72 & 52.7\\
Xception Block 5 & 99.27 & 68.25 & 66.68 & 43.20 & 83.52 & 92.23 & 63.75 & 49.9 \\
MesoInception4 & 97.28 & 59.27 & 60.17 & 47.24 & 65.75 & 83.27 & 62.92 & 54.0 \\
Resnet-18 & 93.90 & 53.22 & 53.45 & 53.69 & 69.98 & 85.40 & 54.77 & 50.8 \\
Xception & 98.60 & 60.15 & 56.84 & 46.12 & 70.07 & 93.61 & 56.79 & 48.5\\
CNN (p=0.1) & 97.78 & 60.08 & 59.73 & 50.87 & 68.67 & 95.16 & 68.15 & 47.4\\
CNN (p=0.5) & 98.16 & 54.02 & 56.06 & 55.99 & 66.98 & 95.03 & 71.50 & 51.9 \\

% \textbf{Our} & \textbf{99.91} & \textbf{85.13} & \textbf{78.27} & \textbf{78.12} & \textbf{86.18} & \textbf{98.56} & \textbf{76.40} & \textbf{68.06} \\ 
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 98.44 & \textbf{75.22} & 67.27 & \textbf{61.47} & \textbf{84.96} & \textbf{97.17} & 68.12 & \textbf{57.95} \\ 
% \textbf{After Bug fix 5 epochs} & 98.80 & \textbf{76.35} & 68.75 & 57.74 & \textbf{85.87} & \textbf{97.03} & 68.68 & \textbf{56.03} \\
\hline
% \textbf{After Bug fix 1 epoch dual} &97.15 & 70.92 & 62.93 & 57.48 & 76.68 & 82.96 & 66.09 & 55.86 \\

% \textbf{After Bug fix with margin} & 98.92 & 74.95 & 64.95 & 58.04 & \textbf{83.96} & \textbf{97.00} & 71.06 & \textbf{56.94}  \\
% \textbf{Projection Components: 300 PCA score} &
% 99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} \\
\textbf{\bf Ours} &
99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} \\
\end{tabular}

\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{Train on Face2Face}} & \multicolumn{4}{|c|}{\textbf{Train on FaceSwap}} & \multicolumn{3}{|c|}{\textbf{$CoV^{-1}$}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ \\
\hline
Resnet Layer 1 & 84.39 & 79.72 & 97.66 & 60.53 & 59.49 & 52.56 & 62.00 & 97.1 & 73.18 & 15.54 & 4.71 \\
Xception Block 1 & 77.65 & 80.88 & 93.84 & 61.62 & 53.14 & 49.24 & 56.89 & 82.8 & 68.75 & \textbf{14.11} & 4.87\\
Xception Block 2 & 84.04 & 79.51 & 97.40 & 63.21 & 58.39 & 51.65 & 61.73 & 92.5 & 72.02 & 15.07 & 4.78 \\
Xception Block 3 & 76.10 & 74.77 & 97.33 & 63.10 & 61.77 & 53.44 & 61.34 & 96.0& 71.14 & 15.08 & 4.72 \\
Xception Block 4 & 67.18 & 61.72 & 97.19 & 63.04 & 61.33 & 52.02 & 59.45 & 96.5 & 70.85 & 15.57 & 4.55 \\
Xception Block 5 & 81.25 & 61.91 & 96.45 & 55.15 & 57.14 & 47.39 & 54.68 & 95.5 & 69.77 & 18.34 & 3.80 \\
MesoInception4 & 67.53 & 55.17 & 92.27 & 54.06 & 50.64 & 48.87 & 56.15 & 93.8 & 65.52 & 16.22 & 4.04\\
Resnet-18 & 55.43 & 52.57 & 93.27 & 53.39 &  61.03 & 51.66 & 52.56 & 91.4 & 64.16 & 16.20 & 3.96 \\
Xception & 66.12 & 56.07 & 97.41 & 53.15 & 53.86 & 50.00 & 56.55 & 96.8 & 66.29 & 18.43 & 3.60\\
CNN (p=0.1) & 65.76 & 64.81 & 98.40 & 59.48 & 59.19 & 53.50 & 63.07 & 99.0 & 69.44 & 17.19 & 4.04 \\
CNN (p=0.5) & 65.43 & 60.36 & 97.94 & 63.52 & 60.19 & 52.11 & 59.81 & 98.2 & 69.20 & 17.04 & 4.06\\


% \textbf{Our} & \textbf{88.24} & \textbf{82.20} & \textbf{99.99} & \textbf{81.75} & \textbf{87.63} & \textbf{72.93} & \textbf{72.67} & \textbf{99.97} \\
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 67.54 & 62.68 & 98.11 & 63.33 & \textbf{62.50} & \textbf{60.82} & \textbf{65.23} & 98.91 \\ 
% \textbf{After Bug fix 5 epochs} & 67.20 & 61.20 & \textbf{98.68} & 59.24 & 59.61 & \textbf{57.69} & \textbf{63.21} & \textbf{99.75} \\
 
% \textbf{After Bug fix 1 epoch dual} & 74.88 & 62.42 & 98.49 & 60.88 & 58.81 & 55.85 & 59.47 & 78.60 \\
% \textbf{After Bug fix with margin} & 74.81 & 65.83 & 98.26 & 59.76 & \textbf{66.09} & \textbf{60.96} & \textbf{64.30} & \textbf{99.08}  \\
% \textbf{Projection Components: 300 PCA score} & 77.43 & 66.78 & 98.26 & 61.49 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} \\
\textbf{\bf Ours} & 77.43 & 66.78 & 98.26 & 61.49 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} & \textbf{75.57} & 14.94 & \textbf{5.06} \\
\hline

\end{tabular}
\caption{\textbf{Deepfake Detection} Average precision on FaceForensics++~\cite{roessler2019faceforensicspp} datasets when trained on one manipulation and tested against all four. Our model is ranked first in the highest frequency. Our method is ranked first in 10 times, while the second best models Resnet Layer 1 and CNN(p=0.5) achieved the highest AP merely two times. Consequently, we rank first in the Deepfake and FaceSwap datasets in the $CoV^{-1}$ score.}
\label{tab:AveragePrecisionFaceForensics}


\end{table*}

==> Tables/OLD_Tables/AveragePrecisionFaceForensics.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{Train on Deepfakes}} & \multicolumn{4}{|c|}{\textbf{Train on Neural Textures}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} \\
\hline
\hline
Resnet Layer 1 & 98.97 & 74.99 & 71.74 & 57.15 & 70.32 & 86.93 & 65.04 & 52.37 \\ 
Xception Block 1 & 92.95 & 70.52 & 65.94 & 52.83 & 66.30 & 80.72 & 62.65 & 52.05 \\ 
Xception Block 2 & 98.04 & 70.28 & 67.48 & 56.04 & 69.31 & 85.75 & 64.27 & 52.70 \\ 
Xception Block 3 & 99.41 & 67.58 & 63.62 & 57.97 & 67.62 & 85.44 & 60.71 & 52.07 \\ 
Xception Block 4 & 99.14 & 68.91 & 70.36 & 58.74 & 73.65 & 90.97 & 60.72 & 52.79 \\ 
Xception Block 5 & 99.27 & 68.25 & 66.68 & 43.20 & 83.52 & 92.23 & 63.75 & 49.94 \\ 
MesoInception4 & 97.28 & 59.27 & 60.17 & 47.24 & 65.75 & 83.27 & 62.92 & 54.03 \\ 
Resnet-18 & 93.90 & 53.22 & 53.45 & 53.69 & 69.98 & 85.40 & 54.77 & 50.89 \\ 
Xception & 98.60 & 60.15 & 56.84 & 46.12 & 70.07 & 93.61 & 56.79 & 48.55 \\ 
CNN (p=0.1) & 97.78 & 60.08 & 59.73 & 50.87 & 68.67 & 95.16 & 68.15 & 47.43 \\ 
CNN (p=0.5) & 98.16 & 54.02 & 56.06 & 55.99 & 66.98 & 95.03 & 71.50 & 51.93 \\ 
% \textbf{Our} & \textbf{99.91} & \textbf{85.13} & \textbf{78.27} & \textbf{78.12} & \textbf{86.18} & \textbf{98.56} & \textbf{76.40} & \textbf{68.06} \\ 
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 98.44 & \textbf{75.22} & 67.27 & \textbf{61.47} & \textbf{84.96} & \textbf{97.17} & 68.12 & \textbf{57.95} \\ 
% \textbf{After Bug fix 5 epochs} & 98.80 & \textbf{76.35} & 68.75 & 57.74 & \textbf{85.87} & \textbf{97.03} & 68.68 & \textbf{56.03} \\
\hline
% \textbf{After Bug fix 1 epoch dual} &97.15 & 70.92 & 62.93 & 57.48 & 76.68 & 82.96 & 66.09 & 55.86 \\

% \textbf{After Bug fix with margin} & 98.92 & 74.95 & 64.95 & 58.04 & \textbf{83.96} & \textbf{97.00} & 71.06 & \textbf{56.94}  \\
% \textbf{Projection Components: 300 PCA score} &
% 99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} \\
\textbf{\bf Ours} &
99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} \\


\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{Train on Face2Face}} & \multicolumn{4}{|c|}{\textbf{Train on FaceSwap}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} \\
\hline
\hline
Resnet Layer 1 & 84.39 & 79.72 & 97.66 & 60.53 & 59.49 & 52.56 & 62.00 & 97.13 \\ 
Xception Block 1 & 77.65 & 80.88 & 93.84 & 61.62 & 53.14 & 49.24 & 56.89 & 82.89 \\ 
Xception Block 2 & 84.04 & 79.51 & 97.40 & 63.21 & 58.39 & 51.65 & 61.73 & 92.58 \\ 
Xception Block 3 & 76.10 & 74.77 & 97.33 & 63.10 & 61.77 & 53.44 & 61.34 & 96.06 \\ 
Xception Block 4 & 67.18 & 61.72 & 97.19 & 63.04 & 61.33 & 52.02 & 59.45 & 96.56 \\ 
Xception Block 5 & 81.25 & 61.91 & 96.45 & 55.15 & 57.14 & 47.39 & 54.68 & 95.57 \\ 
MesoInception4 & 67.53 & 55.17 & 92.27 & 54.06 & 50.64 & 48.87 & 56.15 & 93.81 \\ 
Resnet-18 & 55.43 & 52.57 & 93.27 & 53.39 & 61.03 & 51.66 & 52.56 & 91.49 \\ 
Xception & 66.12 & 56.07 & 97.41 & 53.15 & 53.86 & 50.00 & 56.55 & 96.84 \\ 
CNN (p=0.1) & 65.76 & 64.81 & 98.40 & 59.48 & 59.19 & 53.50 & 63.07 & 99.02 \\ 
CNN (p=0.5) & 65.43 & 60.36 & 97.94 & 63.52 & 60.19 & 52.11 & 59.81 & 98.25 \\ 
% \textbf{Our} & \textbf{88.24} & \textbf{82.20} & \textbf{99.99} & \textbf{81.75} & \textbf{87.63} & \textbf{72.93} & \textbf{72.67} & \textbf{99.97} \\
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 67.54 & 62.68 & 98.11 & 63.33 & \textbf{62.50} & \textbf{60.82} & \textbf{65.23} & 98.91 \\ 
% \textbf{After Bug fix 5 epochs} & 67.20 & 61.20 & \textbf{98.68} & 59.24 & 59.61 & \textbf{57.69} & \textbf{63.21} & \textbf{99.75} \\
 
% \textbf{After Bug fix 1 epoch dual} & 74.88 & 62.42 & 98.49 & 60.88 & 58.81 & 55.85 & 59.47 & 78.60 \\
% \textbf{After Bug fix with margin} & 74.81 & 65.83 & 98.26 & 59.76 & \textbf{66.09} & \textbf{60.96} & \textbf{64.30} & \textbf{99.08}  \\
% \textbf{Projection Components: 300 PCA score} & 77.43 & 66.78 & 98.26 & 61.49 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} \\
\textbf{\bf Ours} & 77.43 & 66.78 & 98.26 & 61.49 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} \\

\hline
\end{tabular}
\end{center}
\caption{\textbf{Deepfake Detection} Average precision on FaceForensics++~\cite{roessler2019faceforensicspp} datasets when trained on one manipulation and tested against all four. Our model is ranked first in the highest frequency. Our method is ranked first in 8 times, while the second best models Resnet Layer 1 and CNN(p=0.5) achieved the highest AP merely two times.}
\label{tab:AveragePrecisionFaceForensics}
\end{table*}

==> Tables/OLD_Tables/DeepfakeCoV.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} \\
\hline
\hline
Resnet Layer 1 & 5.04 & 5.54 & 6.05 & 3.92 \\
Xception Block 1 & 4.88 & \textbf{6.38} & \textbf{6.84} & 4.59 \\
Xception Block 2 & 4.73 & 5.72 & 6.63 & 4.20 \\
Xception Block 3 & 4.48 & 5.42 & 6.30 & 4.14 \\
Xception Block 4 & 4.94 & 4.81 & 4.98 & 3.91 \\
Xception Block 5 & 3.48 & 4.37 & 4.53 & 3.40 \\
MesoInception4 & 3.52 & 6.27 & 4.37 & 3.40 \\
Resnet-18 & 3.63 & 4.78 & 3.72 & 3.97 \\
Xception & 3.30 & 3.95 & 3.89 & 3.40 \\
CNN (p=0.1) & 3.71 & 4.12 & 4.69 & 3.85 \\
CNN (p=0.5) & 3.56 & 4.61 & 4.73 & 3.76 \\
\hline
\hline
\textbf{BUG Ours} & \textbf{9.63} & \textbf{11.96} & \textbf{7.33} & \textbf{7.24} \\
\textbf{Ours} & \textbf{5.05} & 5.17 & 5.40 & \textbf{4.79} \\
\hline
\end{tabular}
\caption{\textbf{Deepfake Detection} Coefficient of Variation rank of~\ref{tab:AveragePrecisionFaceForensics}. Each column corresponds to the dataset used to train each model (row). The entry is the CoV score of all four Average Precision scores for the four FF++ manipulations.}
\label{tab:my_label}
\end{table}

==> Tables/OLD_Tables/DeepfakeGlobalCoV.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{|l|c|c|c|}
  \label{tab:DeepfakeGloabalCoV}
\hline
\textbf{Model} & \textbf{mean} & \textbf{std} & \textbf{$CoV^{-1}$}\\
\hline
\hline
Resnet Layer 1 & 73.18 & 15.54 & 4.71 \\
Xception Block 1 & 68.75 & \textbf{14.11} & 4.87 \\
Xception Block 2 & 72.02 & 15.07 & 4.78 \\
Xception Block 3 & 71.14 & 15.08 & 4.72 \\
Xception Block 4 & 70.85 & 15.57 & 4.55 \\
Xception Block 5 & 69.77 & 18.34 & 3.80 \\
MesoInception4 & 65.52 & 16.22 & 4.04 \\
Resnet-18 & 64.16 & 16.20 & 3.96 \\
Xception & 66.29 & 18.43 & 3.60 \\
CNN (p=0.1) & 69.44 & 17.19 & 4.04 \\
CNN (p=0.5) & 69.20 & 17.04 & 4.06 \\
\hline 
\hline
Ours & \textbf{75.57} & 14.94 & \textbf{5.06} \\


\end{tabular}
\caption{\textbf{Deepfake Detection} Coefficient of Variation rank of~\ref{tab:AveragePrecisionFaceForensics}. The Coefficient of Variance is computed across all Average Precision scores.}

\end{table}

==> Tables/OLD_Tables/DeepfakeTableWithCov.tex <==

\begin{table*}[h]
\parbox[c]{.45\linewidth}{
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{7}{|c|}{\textbf{Train on Deepfakes}} & \multicolumn{7}{|c|}{\textbf{Train on Neural Textures}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ \\
\hline
\hline
Resnet Layer 1 & 98.97 & 74.99 & 71.74 & 57.15 & 75.71 & 15.01 & 5.04 & 70.32 & 86.93 & 65.04 & 52.3 & 68.65 & 12.42 & 5.53 \\
Xception Block 1 & 92.95 & 70.52 & 65.94 & 52.83 & 70.56 & 14.47 & 4.88 & 66.30 & 80.72 & 62.65 & 52.0 & 65.42 & 10.28 & 6.36 \\
Xception Block 2 & 98.04 & 70.28 & 67.48 & 56.04 & 72.96 & 15.43 & 4.73 & 69.31 & 85.75 & 64.27 & 52.7 & 68.01 & 11.88 & 5.72 \\
Xception Block 3 & 99.41 & 67.58 & 63.62 & 57.97 & 72.15 & 16.11 & 4.48 & 67.62 & 85.44 & 60.71 & 52.0 & 66.44 & 12.29 & 5.41 \\
Xception Block 4 & 99.14 & 68.91 & 70.36 & 58.74 & 74.29 & 15.03 & 4.94 & 73.65 & 90.97 & 60.72 & 52.7 & 69.51 & 14.47 & 4.80 \\
Xception Block 5 & 99.27 & 68.25 & 66.68 & 43.20 & 69.35 & 19.92 & 3.48 & 83.52 & 92.23 & 63.75 & 49.9 & 72.35 & 16.57 & 4.37 \\
MesoInception4 & 97.28 & 59.27 & 60.17 & 47.24 & 65.99 & 18.77 & 3.52 & 65.75 & 83.27 & 62.92 & 54.0 & 66.48 & 10.62 & 6.26 \\
Resnet-18 & 93.90 & 53.22 & 53.45 & 53.69 & 63.56 & 17.51 & 3.63 & 69.98 & 85.40 & 54.77 & 50.8 & 65.24 & 13.67 & 4.77 \\
Xception & 98.60 & 60.15 & 56.84 & 46.12 & 65.43 & 19.84 & 3.30 & 70.07 & 93.61 & 56.79 & 48.5 & 67.24 & 17.06 & 3.94 \\
CNN (p=0.1) & 97.78 & 60.08 & 59.73 & 50.87 & 67.11 & 18.09 & 3.71 & 68.67 & 95.16 & 68.15 & 47.4 & 69.84 & 16.95 & 4.12 \\
CNN (p=0.5) & 98.16 & 54.02 & 56.06 & 55.99 & 66.06 & 18.55 & 3.56 & 66.98 & 95.03 & 71.50 & 51.9 & 71.35 & 15.48 & 4.61 \\

% \textbf{Our} & \textbf{99.91} & \textbf{85.13} & \textbf{78.27} & \textbf{78.12} & \textbf{86.18} & \textbf{98.56} & \textbf{76.40} & \textbf{68.06} \\ 
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 98.44 & \textbf{75.22} & 67.27 & \textbf{61.47} & \textbf{84.96} & \textbf{97.17} & 68.12 & \textbf{57.95} \\ 
% \textbf{After Bug fix 5 epochs} & 98.80 & \textbf{76.35} & 68.75 & 57.74 & \textbf{85.87} & \textbf{97.03} & 68.68 & \textbf{56.03} \\
\hline
% \textbf{After Bug fix 1 epoch dual} &97.15 & 70.92 & 62.93 & 57.48 & 76.68 & 82.96 & 66.09 & 55.86 \\

% \textbf{After Bug fix with margin} & 98.92 & 74.95 & 64.95 & 58.04 & \textbf{83.96} & \textbf{97.00} & 71.06 & \textbf{56.94}  \\
% \textbf{Projection Components: 300 PCA score} &
% 99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} \\
\textbf{\bf Ours} &
99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & 75.67 & 15.00 & 5.05 & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} & 77.66 & 15.03 & 5.17 \\


\hline
\multicolumn{1}{|c|}{}& \multicolumn{7}{|c|}{\textbf{Train on Face2Face}} & \multicolumn{7}{|c|}{\textbf{Train on FaceSwap}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ \\
\hline
\hline
Resnet Layer 1 & 84.39 & 79.72 & 97.66 & 60.53 & 80.57 & 13.31 & 6.05 & 59.49 & 52.56 & 62.00 & 97.1 & 67.79 & 17.27 & 3.92 \\
Xception Block 1 & 77.65 & 80.88 & 93.84 & 61.62 & 78.50 & 11.47 & 6.84 & 53.14 & 49.24 & 56.89 & 82.8 & 60.52 & 13.15 & 4.60 \\
Xception Block 2 & 84.04 & 79.51 & 97.40 & 63.21 & 81.04 & 12.22 & 6.63 & 58.39 & 51.65 & 61.73 & 92.5 & 66.07 & 15.69 & 4.21 \\
Xception Block 3 & 76.10 & 74.77 & 97.33 & 63.10 & 77.83 & 12.34 & 6.30 & 61.77 & 53.44 & 61.34 & 96.0 & 68.14 & 16.42 & 4.15 \\
Xception Block 4 & 67.18 & 61.72 & 97.19 & 63.04 & 72.28 & 14.52 & 4.98 & 61.33 & 52.02 & 59.45 & 96.5 & 67.33 & 17.20 & 3.91 \\
Xception Block 5 & 81.25 & 61.91 & 96.45 & 55.15 & 73.69 & 16.26 & 4.53 & 57.14 & 47.39 & 54.68 & 95.5 & 63.68 & 18.72 & 3.40 \\
MesoInception4 & 67.53 & 55.17 & 92.27 & 54.06 & 67.26 & 15.38 & 4.37 & 50.64 & 48.87 & 56.15 & 93.8 & 62.36 & 18.35 & 3.40 \\
Resnet-18 & 55.43 & 52.57 & 93.27 & 53.39 & 63.66 & 17.12 & 3.72 & 61.03 & 51.66 & 52.56 & 91.4 & 64.16 & 16.14 & 3.97 \\
Xception & 66.12 & 56.07 & 97.41 & 53.15 & 68.19 & 17.54 & 3.89 & 53.86 & 50.00 & 56.55 & 96.8 & 64.30 & 18.91 & 3.40 \\
CNN (p=0.1) & 65.76 & 64.81 & 98.40 & 59.48 & 72.11 & 15.36 & 4.69 & 59.19 & 53.50 & 63.07 & 99.0 & 68.69 & 17.83 & 3.85 \\
CNN (p=0.5) & 65.43 & 60.36 & 97.94 & 63.52 & 71.81 & 15.19 & 4.73 & 60.19 & 52.11 & 59.81 & 98.2 & 67.58 & 17.97 & 3.76 \\


% \textbf{Our} & \textbf{88.24} & \textbf{82.20} & \textbf{99.99} & \textbf{81.75} & \textbf{87.63} & \textbf{72.93} & \textbf{72.67} & \textbf{99.97} \\
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 67.54 & 62.68 & 98.11 & 63.33 & \textbf{62.50} & \textbf{60.82} & \textbf{65.23} & 98.91 \\ 
% \textbf{After Bug fix 5 epochs} & 67.20 & 61.20 & \textbf{98.68} & 59.24 & 59.61 & \textbf{57.69} & \textbf{63.21} & \textbf{99.75} \\
 
% \textbf{After Bug fix 1 epoch dual} & 74.88 & 62.42 & 98.49 & 60.88 & 58.81 & 55.85 & 59.47 & 78.60 \\
% \textbf{After Bug fix with margin} & 74.81 & 65.83 & 98.26 & 59.76 & \textbf{66.09} & \textbf{60.96} & \textbf{64.30} & \textbf{99.08}  \\
% \textbf{Projection Components: 300 PCA score} & 77.43 & 66.78 & 98.26 & 61.49 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} \\
\textbf{\bf Ours} & 77.43 & 66.78 & 98.26 & 61.49 & 75.99 & 14.08 & 5.40 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} & 72.97 & 15.24 & 4.79 \\
\hline

\end{tabular}
\caption{\textbf{Deepfake Detection} Average precision on FaceForensics++~\cite{roessler2019faceforensicspp} datasets when trained on one manipulation and tested against all four. Our model is ranked first in the highest frequency. Our method is ranked first in 8 times, while the second best models Resnet Layer 1 and CNN(p=0.5) achieved the highest AP merely two times.}
\label{tab:AveragePrecisionFaceForensics}
}
\hfill
\parbox[c]{.35\linewidth}{
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} \\
\hline
\hline
Resnet Layer 1 & 5.04 & 5.54 & 6.05 & 3.92 \\
Xception Block 1 & 4.88 & \textbf{6.38} & \textbf{6.84} & 4.59 \\
Xception Block 2 & 4.73 & 5.72 & 6.63 & 4.20 \\
Xception Block 3 & 4.48 & 5.42 & 6.30 & 4.14 \\
Xception Block 4 & 4.94 & 4.81 & 4.98 & 3.91 \\
Xception Block 5 & 3.48 & 4.37 & 4.53 & 3.40 \\
MesoInception4 & 3.52 & 6.27 & 4.37 & 3.40 \\
Resnet-18 & 3.63 & 4.78 & 3.72 & 3.97 \\
Xception & 3.30 & 3.95 & 3.89 & 3.40 \\
CNN (p=0.1) & 3.71 & 4.12 & 4.69 & 3.85 \\
CNN (p=0.5) & 3.56 & 4.61 & 4.73 & 3.76 \\
\hline
\hline
\textbf{BUG Ours} & \textbf{9.63} & \textbf{11.96} & \textbf{7.33} & \textbf{7.24} \\
\textbf{Ours} & \textbf{5.05} & 5.17 & 5.40 & \textbf{4.79} \\
\hline
\end{tabular}
\caption{\textbf{Deepfake Detection} Coefficient of Variation rank of~\ref{tab:AveragePrecisionFaceForensics}. Each column corresponds to the dataset used to train each model (row). The entry is the CoV score of all four Average Precision scores for the four FF++ manipulations.}
}
\label{tab:my_label}
\end{table*}


==> Tables/OLD_Tables/DeepfakeWithCoVTablesOLD.tex <==

\begin{table*}[]
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{7}{|c|}{\textbf{Train on Deepfakes}} & \multicolumn{7}{|c|}{\textbf{Train on Neural Textures}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ \\
\hline
\hline
Resnet Layer 1 & 98.97 & 74.99 & 71.74 & 57.15 & \textbf{75.71} & 15.01 & 5.04 & 70.32 & 86.93 & 65.04 & 52.3 & 68.65 & 12.42 & 5.53 \\
Xception Block 1 & 92.95 & 70.52 & 65.94 & 52.83 & 70.56 & \textbf{14.47} & 4.88 & 66.30 & 80.72 & 62.65 & 52.0 & 65.42 & \textbf{10.28} & \textbf{6.36} \\
Xception Block 2 & 98.04 & 70.28 & 67.48 & 56.04 & 72.96 & 15.43 & 4.73 & 69.31 & 85.75 & 64.27 & 52.7 & 68.01 & 11.88 & 5.72 \\
Xception Block 3 & 99.41 & 67.58 & 63.62 & 57.97 & 72.15 & 16.11 & 4.48 & 67.62 & 85.44 & 60.71 & 52.0 & 66.44 & 12.29 & 5.41 \\
Xception Block 4 & 99.14 & 68.91 & 70.36 & 58.74 & 74.29 & 15.03 & 4.94 & 73.65 & 90.97 & 60.72 & 52.7 & 69.51 & 14.47 & 4.80 \\
Xception Block 5 & 99.27 & 68.25 & 66.68 & 43.20 & 69.35 & 19.92 & 3.48 & 83.52 & 92.23 & 63.75 & 49.9 & 72.35 & 16.57 & 4.37 \\
MesoInception4 & 97.28 & 59.27 & 60.17 & 47.24 & 65.99 & 18.77 & 3.52 & 65.75 & 83.27 & 62.92 & 54.0 & 66.48 & 10.62 & 6.26 \\
Resnet-18 & 93.90 & 53.22 & 53.45 & 53.69 & 63.56 & 17.51 & 3.63 & 69.98 & 85.40 & 54.77 & 50.8 & 65.24 & 13.67 & 4.77 \\
Xception & 98.60 & 60.15 & 56.84 & 46.12 & 65.43 & 19.84 & 3.30 & 70.07 & 93.61 & 56.79 & 48.5 & 67.24 & 17.06 & 3.94 \\
CNN (p=0.1) & 97.78 & 60.08 & 59.73 & 50.87 & 67.11 & 18.09 & 3.71 & 68.67 & 95.16 & 68.15 & 47.4 & 69.84 & 16.95 & 4.12 \\
CNN (p=0.5) & 98.16 & 54.02 & 56.06 & 55.99 & 66.06 & 18.55 & 3.56 & 66.98 & 95.03 & 71.50 & 51.9 & 71.35 & 15.48 & 4.61 \\

% \textbf{Our} & \textbf{99.91} & \textbf{85.13} & \textbf{78.27} & \textbf{78.12} & \textbf{86.18} & \textbf{98.56} & \textbf{76.40} & \textbf{68.06} \\ 
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 98.44 & \textbf{75.22} & 67.27 & \textbf{61.47} & \textbf{84.96} & \textbf{97.17} & 68.12 & \textbf{57.95} \\ 
% \textbf{After Bug fix 5 epochs} & 98.80 & \textbf{76.35} & 68.75 & 57.74 & \textbf{85.87} & \textbf{97.03} & 68.68 & \textbf{56.03} \\
\hline
% \textbf{After Bug fix 1 epoch dual} &97.15 & 70.92 & 62.93 & 57.48 & 76.68 & 82.96 & 66.09 & 55.86 \\

% \textbf{After Bug fix with margin} & 98.92 & 74.95 & 64.95 & 58.04 & \textbf{83.96} & \textbf{97.00} & 71.06 & \textbf{56.94}  \\
% \textbf{Projection Components: 300 PCA score} &
% 99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} \\
\textbf{\bf Ours} &
99.14 & \textbf{77.17} & 67.38 & \textbf{59.00} & 75.67 & 15.00 & \textbf{5.05} & \textbf{84.88} & \textbf{97.26} & \textbf{71.59} & \textbf{56.92} & \textbf{77.66} & 15.03 & 5.17 \\


\hline
\multicolumn{1}{|c|}{}& \multicolumn{7}{|c|}{\textbf{Train on Face2Face}} & \multicolumn{7}{|c|}{\textbf{Train on FaceSwap}} \\

\textbf{Model} & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ & \textbf{DF} & \textbf{NT} & \textbf{F2F} & \textbf{FS} & mean & std & $CoV^{-1}$ \\
\hline
\hline
Resnet Layer 1 & 84.39 & 79.72 & 97.66 & 60.53 & \textbf{80.57} & 13.31 & 6.05 & 59.49 & 52.56 & 62.00 & 97.1 & 67.79 & 17.27 & 3.92 \\
Xception Block 1 & 77.65 & 80.88 & 93.84 & 61.62 & 78.50 & \textbf{11.47} & \textbf{6.84} & 53.14 & 49.24 & 56.89 & 82.8 & 60.52 & \textbf{13.15} & 4.60 \\
Xception Block 2 & 84.04 & 79.51 & 97.40 & 63.21 & 81.04 & 12.22 & 6.63 & 58.39 & 51.65 & 61.73 & 92.5 & 66.07 & 15.69 & 4.21 \\
Xception Block 3 & 76.10 & 74.77 & 97.33 & 63.10 & 77.83 & 12.34 & 6.30 & 61.77 & 53.44 & 61.34 & 96.0 & 68.14 & 16.42 & 4.15 \\
Xception Block 4 & 67.18 & 61.72 & 97.19 & 63.04 & 72.28 & 14.52 & 4.98 & 61.33 & 52.02 & 59.45 & 96.5 & 67.33 & 17.20 & 3.91 \\
Xception Block 5 & 81.25 & 61.91 & 96.45 & 55.15 & 73.69 & 16.26 & 4.53 & 57.14 & 47.39 & 54.68 & 95.5 & 63.68 & 18.72 & 3.40 \\
MesoInception4 & 67.53 & 55.17 & 92.27 & 54.06 & 67.26 & 15.38 & 4.37 & 50.64 & 48.87 & 56.15 & 93.8 & 62.36 & 18.35 & 3.40 \\
Resnet-18 & 55.43 & 52.57 & 93.27 & 53.39 & 63.66 & 17.12 & 3.72 & 61.03 & 51.66 & 52.56 & 91.4 & 64.16 & 16.14 & 3.97 \\
Xception & 66.12 & 56.07 & 97.41 & 53.15 & 68.19 & 17.54 & 3.89 & 53.86 & 50.00 & 56.55 & 96.8 & 64.30 & 18.91 & 3.40 \\
CNN (p=0.1) & 65.76 & 64.81 & 98.40 & 59.48 & 72.11 & 15.36 & 4.69 & 59.19 & 53.50 & 63.07 & 99.0 & 68.69 & 17.83 & 3.85 \\
CNN (p=0.5) & 65.43 & 60.36 & 97.94 & 63.52 & 71.81 & 15.19 & 4.73 & 60.19 & 52.11 & 59.81 & 98.2 & 67.58 & 17.97 & 3.76 \\


% \textbf{Our} & \textbf{88.24} & \textbf{82.20} & \textbf{99.99} & \textbf{81.75} & \textbf{87.63} & \textbf{72.93} & \textbf{72.67} & \textbf{99.97} \\
\hline
\hline
% \textbf{After Bug fix 1 epoch} & 67.54 & 62.68 & 98.11 & 63.33 & \textbf{62.50} & \textbf{60.82} & \textbf{65.23} & 98.91 \\ 
% \textbf{After Bug fix 5 epochs} & 67.20 & 61.20 & \textbf{98.68} & 59.24 & 59.61 & \textbf{57.69} & \textbf{63.21} & \textbf{99.75} \\
 
% \textbf{After Bug fix 1 epoch dual} & 74.88 & 62.42 & 98.49 & 60.88 & 58.81 & 55.85 & 59.47 & 78.60 \\
% \textbf{After Bug fix with margin} & 74.81 & 65.83 & 98.26 & 59.76 & \textbf{66.09} & \textbf{60.96} & \textbf{64.30} & \textbf{99.08}  \\
% \textbf{Projection Components: 300 PCA score} & 77.43 & 66.78 & 98.26 & 61.49 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} \\
\textbf{\bf Ours} & 77.43 & 66.78 & 98.26 & 61.49 & 75.99 & 14.08 & 5.40 & \textbf{64.83} & \textbf{61.47} & \textbf{66.41} & \textbf{99.19} & \textbf{72.97} & 15.24 & \textbf{4.79} \\
\hline

\end{tabular}
\caption{\textbf{Deepfake Detection} Average precision on FaceForensics++~\cite{roessler2019faceforensicspp} datasets when trained on one manipulation and tested against all four. Our model is ranked first in the highest frequency. Our method is ranked first in 10 times, while the second best models Resnet Layer 1 and CNN(p=0.5) achieved the highest AP merely two times. Consequently, we rank first in the Deepfake and FaceSwap datasets in the $CoV^{-1}$ score.}
\label{tab:AveragePrecisionFaceForensics}


\end{table*}

==> Tables/OLD_Tables/SyntheticImageTableWithCoV.tex <==

\begin{table*}[h]
\label{tab:SyntheticImagesAveragePrecisionWithCoV}
\parbox[c]{.6\linewidth}{
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{CelebA-HQ dataset}} & \multicolumn{3}{|c|}{\textbf{FFHQ dataset}} & \multicolumn{3}{|c|}{\textbf{CoV}} \\

\textbf{Model } & \textbf{PGAN} & \textbf{SGAN} & \textbf{Glow} & \textbf{GMM} & \textbf{PGAN} & \textbf{SGAN} & \textbf{SGAN2} &  \textbf{mean} &  \textbf{std} & \textbf{CoV^-1}\\
\hline
\hline
Resnet Layer 1 & 100.0 & 97.22 & 72.80 & 80.69 & 99.81 & 72.91 & 71.81 & 82.54 & 11.69 & 7.06 \\
Xception Block 1 & 100.0 & 98.68 & 95.48 & 76.21 & 99.68 & 81.35 & 77.40 & 88.13 & 10.02 & 8.80 \\
Xception Block 2 & 100.0 & 99.99 & 67.49 & \textbf{91.38} & \textbf{100.0} & 90.12 & 90.85 & 89.97 & 10.87 & 8.28 \\
Xception Block 3 & 100.0 & \textbf{100.0} & 74.98 & 80.96 & 100.0 & 92.91 & \textbf{91.45} & 90.05 & 9.29 & 9.69 \\
Xception Block 4 & 100.0 & 99.99 & 66.79 & 42.82 & 100.0 & \textbf{95.85} & 90.62 & 82.68 & 21.12 & 3.91 \\
Xception Block 5 & 100.0 & 100.0 & 60.44 & 48.92 & 100.0 & 93.09 & 89.08 & 81.92 & 19.92 & 4.11 \\
MesoInception4 & 100.0 & 97.90 & 49.72 & 45.98 & 98.71 & 80.57 & 71.27 & 74.02 & 20.84 & 3.55 \\
Resnet-18 & 100.0 & 64.80 & 47.06 & 54.69 & 79.20 & 51.15 & 52.37 & 58.21 & 10.84 & 5.37 \\
Xception & 100.0 & 99.75 & 55.85 & 40.98 & 99.94 & 85.69 & 74.33 & 76.09 & 21.86 & 3.48 \\
CNN (p=0.1) & 100.0 & 98.41 & 90.46 & 50.65 & 99.95 & 90.48 & 85.27 & 85.87 & 16.53 & 5.20 \\
CNN (p=0.5) & 100.0 & 97.34 & \textbf{97.32} & 73.33 & 99.93 & 88.98 & 84.58 & 90.25 & 9.26 & 9.75 \\

\hline
\hline
Our & 100.00 & 97.06 & 87.82 & 89.19 & 99.77 & 81.15 & 76.22 & 88.54 & \textbf{8.23} & \textbf{10.76} \\
 \\
\hline
\end{tabular}
\caption{\textbf{Synthetic Image Detection} Average precision on different model architectures and an alternative dataset (FFHQ). Excluding our results, all numbers extracted from~\cite{chai2020makes}. As can be seen, our method does not excel in any particular experiment but, as Table~\ref{tab:SyntheticImagesCoVRank} shows, we outperform all other methods, on average.}
\end{center}
}
\hfill
\parbox[c]{.35\linewidth}{
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Model} & \textbf{$CoV ^{-1}: \frac{<AP>}{std(AP)}$}\\
\hline
\hline
Xception & 3.48 \\
MesoInception4 & 3.55 \\
Xception Block 4 & 3.91 \\
Xception Block 5 & 4.11 \\
CNN (p=0.1) & 5.2 \\
Resnet-18 & 5.37 \\
Resnet Layer 1 & 7.06 \\
EfficientNet-V2 & 7.17 \\
Xception++ & 7.53 \\
Xception Block 2 & 8.28 \\
Xception Block 1 & 8.80 \\
Xception Block 3 & 9.69 \\
CNN (p=0.5) & 9.75 \\
\textbf{EfficientNet-V2++} & \textbf{10.47} \\
\hline
\end{tabular}
\caption{\textbf{Synthetic Image Detection} Coefficient of Variation rank for each method for the task of Synthetic image detection. Our method applied to EfficientNet-V2 backbone, \textit{EfficientNet-V2++}, ranks highest on the $CoV^{-1}$ rank for the detection of Synthetic images based on a single train dataset of PGAN. We test ourselves against SGAN, Glow and GMM trained once using CelebA-HQ and second when the GANs are trained against FFHQ dataset. Note that EfficientNet-V2++ ranks $7.17$ with respect to $10.47$ including our architecture change. A similar architecture change boosted the performance of Xception network from $3.48$ to $7.53$.}
}
\end{table*}


==> Tables/OLD_Tables/SyntheticImageTablesOLD.tex <==

\begin{table*}[h]
\label{tab:SyntheticImagesAveragePrecision}
\parbox[c]{.6\linewidth}{
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{CelebA-HQ dataset}} & \multicolumn{3}{|c|}{\textbf{FFHQ dataset}} \\

\textbf{Model } & \textbf{PGAN} & \textbf{SGAN} & \textbf{Glow} & \textbf{GMM} & \textbf{PGAN} & \textbf{SGAN} & \textbf{SGAN2} \\
\hline
\hline
Resnet Layer 1 & 100.0 & 97.22 & 72.80 & 80.69 & 99.81 & 72.91 & 71.81 \\
Xception Block 1 & 100.0 & 98.68 & 95.48 & 76.21 & 99.68 & 81.35 & 77.40 \\
Xception Block 2 & 100.0 & 99.99 & 67.49 & \textbf{91.38} & \textbf{100.0} & 90.12 & 90.85 \\
Xception Block 3 & 100.0 & \textbf{100.0} & 74.98 & 80.96 & 100.0 & 92.91 & \textbf{91.45} \\
Xception Block 4 & 100.0 & 99.99 & 66.79 & 42.82 & 100.0 & \textbf{95.85} & 90.62 \\
Xception Block 5 & 100.0 & 100.0 & 60.44 & 48.92 & 100.0 & 93.09 & 89.08 \\
MesoInception4 & 100.0 & 97.90 & 49.72 & 45.98 & 98.71 & 80.57 & 71.27 \\
Resnet-18 & 100.0 & 64.80 & 47.06 & 54.69 & 79.20 & 51.15 & 52.37 \\
Xception & 100.0 & 99.75 & 55.85 & 40.98 & 99.94 & 85.69 & 74.33 \\
CNN (p=0.1) & 100.0 & 98.41 & 90.46 & 50.65 & 99.95 & 90.48 & 85.27 \\
CNN (p=0.5) & 100.0 & 97.34 & \textbf{97.32} & 73.33 & 99.93 & 88.98 & 84.58 \\
\hline
\hline
\textbf{Our} & 100.00 & 97.06 & 87.82 & 89.19 & 99.77 & 81.15 & 76.22 \\
\hline
\end{tabular}
\caption{\textbf{Synthetic Image Detection} Average precision on different model architectures and an alternative dataset (FFHQ). Excluding our results, all numbers extracted from~\cite{chai2020makes}. As can be seen, our method does not excel in any particular experiment but, as Table~\ref{tab:SyntheticImagesCoVRank} shows, we outperform all other methods, on average.}
\end{center}
}
\hfill
\parbox[c]{.35\linewidth}{
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Model} & \textbf{$CoV ^{-1}: \frac{<AP>}{std(AP)}$}\\
\hline
\hline
Xception & 3.48 \\
MesoInception4 & 3.55 \\
Xception Block 4 & 3.91 \\
Xception Block 5 & 4.11 \\
CNN (p=0.1) & 5.2 \\
Resnet-18 & 5.37 \\
Resnet Layer 1 & 7.06 \\
EfficientNet-V2 & 7.17 \\
Xception++ & 7.53 \\
Xception Block 2 & 8.28 \\
Xception Block 1 & 8.80 \\
Xception Block 3 & 9.69 \\
CNN (p=0.5) & 9.75 \\
\textbf{EfficientNet-V2++} & \textbf{10.47} \\
\hline
\end{tabular}
\caption{\textbf{Synthetic Image Detection} Coefficient of Variation rank for each method for the task of Synthetic image detection. Our method applied to EfficientNet-V2 backbone, \textit{EfficientNet-V2++}, ranks highest on the $CoV^{-1}$ rank for the detection of Synthetic images based on a single train dataset of PGAN. We test ourselves against SGAN, Glow and GMM trained once using CelebA-HQ and second when the GANs are trained against FFHQ dataset. Note that EfficientNet-V2++ ranks $7.17$ with respect to $10.47$ including our architecture change. A similar architecture change boosted the performance of Xception network from $3.48$ to $7.53$.}
}
\end{table*}


==> Tables/OLD_Tables/SyntheticImagesAveragePrecision.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{4}{|c|}{\textbf{Architectures}} & \multicolumn{3}{|c|}{\textbf{FFHQ dataset}} \\

\textbf{Model } & \textbf{PGAN} & \textbf{SGAN} & \textbf{Glow} & \textbf{GMM} & \textbf{PGAN} & \textbf{SGAN} & \textbf{SGAN2} \\
\hline
\hline
Resnet Layer 1 & 100.0 & 97.22 & 72.80 & 80.69 & 99.81 & 72.91 & 71.81 \\
Xception Block 1 & 100.0 & 98.68 & 95.48 & 76.21 & 99.68 & 81.35 & 77.40 \\
Xception Block 2 & 100.0 & 99.99 & 67.49 & \textbf{91.38} & \textbf{100.0} & 90.12 & 90.85 \\
Xception Block 3 & 100.0 & \textbf{100.0} & 74.98 & 80.96 & 100.0 & 92.91 & \textbf{91.45} \\
Xception Block 4 & 100.0 & 99.99 & 66.79 & 42.82 & 100.0 & \textbf{95.85} & 90.62 \\
Xception Block 5 & 100.0 & 100.0 & 60.44 & 48.92 & 100.0 & 93.09 & 89.08 \\
MesoInception4 & 100.0 & 97.90 & 49.72 & 45.98 & 98.71 & 80.57 & 71.27 \\
Resnet-18 & 100.0 & 64.80 & 47.06 & 54.69 & 79.20 & 51.15 & 52.37 \\
Xception & 100.0 & 99.75 & 55.85 & 40.98 & 99.94 & 85.69 & 74.33 \\
CNN (p=0.1) & 100.0 & 98.41 & 90.46 & 50.65 & 99.95 & 90.48 & 85.27 \\
CNN (p=0.5) & 100.0 & 97.34 & \textbf{97.32} & 73.33 & 99.93 & 88.98 & 84.58 \\
\hline
\hline
\textbf{Our} & 100.00 & 97.06 & 87.82 & 89.19 & 99.77 & 81.15 & 76.22 \\
% PGAN            100.00
% celebahq_1sgan   97.06
% celebahq_2glow   87.82
% celebahq_3gmm    89.19
% ffhq_1pgan       99.77
% ffhq_2sgan       81.15
% ffhq_3sgan2      76.22

\hline
\end{tabular}
\end{center}
\caption{\textbf{Synthetic Image Detection} Average precision on different model architectures and an alternative dataset (FFHQ). Excluding our results, all numbers extracted from~\cite{chai2020makes}. As can be seen, our method does not excel in any particular experiment but, as Table~\ref{tab:SyntheticImagesCoVRank} shows, we outperform all other methods, on average.}
\label{tab:SyntheticImagesAveragePrecision}
\end{table*}



==> Tables/OLD_Tables/SyntheticImagesCoVRank.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|}
\hline
\textbf{Model} & \textbf{$CoV ^{-1}: \frac{<AP>}{std(AP)}$}\\
\hline
\hline
Xception & 3.48 \\
MesoInception4 & 3.55 \\
Xception Block 4 & 3.91 \\
Xception Block 5 & 4.11 \\
CNN (p=0.1) & 5.2 \\
Resnet-18 & 5.37 \\
Resnet Layer 1 & 7.06 \\
EfficientNet-V2 & 7.17 \\
Xception++ & 7.53 \\
Xception Block 2 & 8.28 \\
Xception Block 1 & 8.80 \\
Xception Block 3 & 9.69 \\
CNN (p=0.5) & 9.75 \\
\textbf{EfficientNet-V2++} & \textbf{10.47} \\
\hline
\end{tabular}
\end{center}
\caption{\textbf{Synthetic Image Detection} Coefficient of Variation rank for each method for the task of Synthetic image detection. Our method applied to EfficientNet-V2 backbone, \textit{EfficientNet-V2++}, ranks highest on the $CoV^{-1}$ rank for the detection of Synthetic images based on a single train dataset of PGAN. We test ourselves against SGAN, Glow and GMM trained once using CelebA-HQ and second when the GANs are trained against FFHQ dataset. Note that EfficientNet-V2++ ranks $7.17$ with respect to $10.47$ including our architecture change. A similar architecture change boosted the performance of Xception network from $3.48$ to $7.53$.}
\label{tab:SyntheticImagesCoVRank}
\end{table}

==> Tables/OLD_Tables/XceptionBlocksVsOurs.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|}
\hline
\textbf{Model} & \textbf{$CoV ^{-1}: \frac{<AP>}{std(AP)}$}\\
\hline
\hline
Xception & 3.48 \\
Xception Block 4 & 3.91 \\
Xception Block 5 & 4.11 \\
Xception Block 2 & 8.28 \\
Xception Block 1 & 8.80 \\
Xception Block 3 & 9.69 \\
\hline
\textbf{Xception++} & 7.53 \\
\hline
\end{tabular}
\end{center}
\caption{\textbf{Synthetic Image Detection} Coefficient of Variation rank for each Xception Block, the entire Xception network and our method applied for the Xception backbone: \textit{Xception++}. Note that Xception ranks merely $3.48$ with respect to $7.53$ including our architecture change.}
\label{tab:XceptionBlocksVsOurs}
\end{table}
